STLts-Div: Diversified Trace Synthesis from STL Specifications Using MILP (Extended Version)

Modern cyber-physical systems are complex, and requirements are often written in Signal Temporal Logic (STL). Writing the right STL is difficult in practice; engineers benefit from concrete executions that illustrate what a specification actually admits. Trace synthesis addresses this need, but a single witness rarely suffices to understand intent or explore edge cases - diverse satisfying behaviors are far more informative. We introduce diversified trace synthesis: the automatic generation of sets of behaviorally diverse traces that satisfy a given STL formula. Building on a MILP encoding of STL and system model, we formalize three complementary diversification objectives - Boolean distance, random Boolean distance, and value distance - all captured by an objective function and solved iteratively. We implement these ideas in STLts-Div, a lightweight Python tool that integrates with Gurobi.

==> macros.tex <==
% COMMENT CMD
\RequirePackage{todonotes}
% Martin's comment
\newcommand{\martincomment}[1]{\todo[color=Violet!15,size=\small,fancyline,author=Martin]{#1}\xspace}
\newcommand{\martincommentinline}[1]{\todo[inline,color=Violet!15,author=Martin]{#1}\xspace}
% Han's comment
\newcommand{\hancomment}[1]{\todo[color=cyan!15,size=\small,fancyline,author=Han]{#1}\xspace}
\newcommand{\hancommentinline}[1]{\todo[inline,color=cyan!15,author=Han]{#1}\xspace}
% Sota's comment 
\newcommand{\sotacomment}[1]{\todo[color=orange!15,size=\small,fancyline,author=Sota]{#1}\xspace}
\newcommand{\sotacommentinline}[1]{\todo[inline,color=orange!15,author=Sota]{#1}\xspace}
% Jie's comment
\newcommand{\jiecomment}[1]{\todo[color=blue!15,size=\small,fancyline,author=Jie]{#1}\xspace}
\newcommand{\jiecommentinline}[1]{\todo[inline,color=blue!15,author=Jie]{#1}\xspace}
% Zhenya's comment
\newcommand{\zhenyacomment}[1]{\todo[color=NavyBlue!15,size=\small,fancyline,author=Zhenya]{#1}\xspace}
\newcommand{\zhenyacommentinline}[1]{\todo[inline,color=NavyBlue!15,author=Zhenya]{#1}\xspace}
% Ichiro's comment
\newcommand{\ichirocomment}[1]{\todo[color=Maroon!15,size=\small,fancyline,author=Ichiro]{#1}\xspace}
\newcommand{\ichirocommentinline}[1]{\todo[inline,color=Maroon!15,author=Ichiro]{#1}\xspace}

% COLOR
\definecolor{orange9}{RGB}{255, 228, 163}

% COLOR TEXT
\newcommand{\red}[1]{\textcolor{Red}{#1}}

% NUMBER SET
\newcommand{\Reals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\PosReals}{\ensuremath{\mathbb{R}_{> 0}}\xspace}
\newcommand{\NonNegReals}{\ensuremath{\mathbb{R}_{\ge 0}}\xspace}
\newcommand{\Nats}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\Bool}{\ensuremath{\mathbb{B}}\xspace}

% MATHEMATIC SYMBOL
\newcommand{\lddef}{\mathrel{\,:\equiv\,}}
\newcommand{\ddef}{\mathrel{\,:=\,}}
\newcommand{\tif}{\ \textnormal{if}\ }
\newcommand{\assign}{\bm{v}}
\newcommand{\asg}[1][\phi]{\ensuremath{\left\langle{#1}\right\rangle}}
% \newcommand{\hdist}{\ensuremath{\mathop{d_H}\!}}
\newcommand{\pow}[1]{\wp(#1)}
\renewcommand{\vec}[1]{\mathaccent"017E{#1}}
\newcommand{\dif}{\mathop{}\!\mathrm{d}} 
\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
\DeclarePairedDelimiter{\valu}{\langle}{\rangle}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}


%STL SYMBOL
\newcommand{\atoprop}{\ensuremath{p}}
\newcommand{\unt}{\ensuremath{\mathbin{\mathcal{U}}}}
\newcommand{\rels}{\ensuremath{\mathbin{\mathcal{R}}}}
\newcommand{\alw}{\ensuremath{\mathop{\Box}\nolimits}}
\newcommand{\ev}{\ensuremath{\mathop{\Diamond}\nolimits}}


% PERSONAL
\newcommand{\sub}[1][\phi]{\ensuremath{\mathrm{Sub}(#1)}}
\newcommand{\pwlsig}{\varsigma^{\mathrm{pwl}}}
\newcommand{\weakneg}{\mathcal{N}}
\newcommand{\vd}{\ensuremath{\mathop{d_{\mathrm{V}}}}}
\newcommand{\bdist}{\ensuremath{\mathop{d_{\mathrm{B}}}}}
\newcommand{\signal}{\bm{\mathrm{Signal}}}
\newcommand{\tpost}{\textit{t-postfix}}
\newcommand{\model}{\mathcal{M}}
\newcommand{\reftrace}{\ensuremath{\sigma_{\mathrm{ref}}}}
\newcommand{\front}{\ensuremath{\mathrm{f}}}
\newcommand{\rear}{\ensuremath{\mathrm{r}}}
\newcommand{\Deuc}{D_{\mathrm{E}}}

% WRITTING
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\resp}{resp.\xspace}
\newcommand{\etc}{etc.\xspace}

\newcommand{\myparagraph}[1]{\medskip\noindent{\bf #1.}}

\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\U}{\mathcal{U}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Rb}{\mathbb{R}}
\renewcommand{\phi}{\varphi}
\newcommand{\var}[1][\psi]{\def\ArgI{{#1}} \varRelay}
\newcommand{\varRelay}[1][i]{\langle\ArgI\rangle_#1}
\newcommand{\sem}[2]{[\![#1,#2]\!]}

\newcommand{\hl}{\cellcolor{white!20}}
\newcommand{\pie}[1]{%
    \begin{tikzpicture}[scale=.8, baseline=-3pt]
        \draw (0,0) circle (1ex);
        \fill (0,0) -- (90:1ex) arc (90:90-#1:1ex) -- cycle;
    \end{tikzpicture}%
}

\newcommand{\bullseye}{%
  \begin{tikzpicture}[scale=.8, baseline=-3pt]
    \draw (0,0) circle (1ex);     
    \fill (0,0) circle (0.45ex);  
  \end{tikzpicture}%
}

\newcommand{\feature}[2][]{%
    \ifthenelse{\equal{#1}{nohl}}{}{%
        \ifthenelse{\equal{#2}{++}}{\hl}{}%
        \ifthenelse{\equal{#2}{+}}{\hl}{}%
    }%
    \ifthenelse{\equal{#2}{++}}{\pie{360}}{}%
    \ifthenelse{\equal{#2}{+}}{\bullseye}{}%
    \ifthenelse{\equal{#2}{-}}{\pie{0}}{}%
    \ifthenelse{\equal{#2}{--}}{-}{}%
}

\newcommand{\cmark}{\ding{51}}  % ✔
\newcommand{\xmark}{\ding{55}}  % ✘

\newcommand{\dstop}{\ensuremath{\mathtt{DSTOP}}\xspace}
\newcommand{\rnc}{\ensuremath{\mathtt{RNC1}}\xspace}
\newcommand{\rncc}{\ensuremath{\mathtt{RNC2}}\xspace}
\newcommand{\rnccc}{\ensuremath{\mathtt{RNC3}}\xspace}
\newcommand{\nav}{\ensuremath{\mathtt{NAV1}}\xspace}
\newcommand{\navv}{\ensuremath{\mathtt{NAV2}}\xspace}
\newcommand{\iso}{\ensuremath{\mathtt{ISO1}}\xspace}
\newcommand{\isot}{\ensuremath{\mathtt{ISO3}}\xspace}
\newcommand{\isofo}{\ensuremath{\mathtt{ISO4}}\xspace}
\newcommand{\isofi}{\ensuremath{\mathtt{ISO5}}\xspace}
\newcommand{\isosi}{\ensuremath{\mathtt{ISO6}}\xspace}
\newcommand{\isose}{\ensuremath{\mathtt{ISO7}}\xspace}
\newcommand{\isoe}{\ensuremath{\mathtt{ISO8}}\xspace}

\newcommand{\kunit}{\ensuremath{\mathrm{k}}}
\newcommand{\Munit}{\ensuremath{\mathrm{M}}}
\newcommand{\Gunit}{\ensuremath{\mathrm{G}}}

\newcommand{\smallsim}{\mathrel{\raisebox{0.2ex}{$\scriptstyle\sim$}}}

\newcommand{\about}[1]{\ensuremath{\smallsim\!#1}\xspace}
\newcommand{\aboutk}[1]{\ensuremath{\smallsim\!#1\kunit}\xspace}
\newcommand{\aboutm}[1]{\ensuremath{\smallsim\!#1\Munit}\xspace}
\newcommand{\ssec}[1]{(\SI{#1}{s})}
